Preconditioning for a Cahn-Hilliard-Navier-Stokes model for morphology formation in organic solar cells

We present a model for the morphology evolution of printed organic solar cells which occurs during the drying of a mixture of polymer, the non-fullerene acceptor and the solvent. Our model uses a phase field approach coupled to a Navier-Stokes equation describing the macroscopic movement of the fluid. Additionally, we incorporate the evaporation process of the solvent using an Allen-Cahn equation. The model is discretized using a finite-element approach with a semi-implicit discretization in time. The resulting (non)linear systems are coupled and of large dimensionality. We present a preconditioned iterative scheme to solve them robustly with respect to changes in the discretization parameters. We illustrate that the preconditioned solver shows parameter-robust iteration numbers and that the model qualitatively captures the behavior of the film morphology during drying.

==> definitions.tex <==
\usepackage[utf8]{inputenc}
\usepackage{amsmath}
\usepackage{amstext} 
\usepackage{array}
\usepackage{accents}
\usepackage{hyperref}
\usepackage{cleveref}
\usepackage{commath}
\newcommand{\ubar}[1]{\underaccent{\bar}{#1}}
\usepackage{graphicx}
\usepackage{float}
\usepackage[colorinlistoftodos,prependcaption,textsize=tiny]{todonotes}
\usepackage{subcaption}
\usepackage{tikz}
\usepackage{bm}
\usetikzlibrary{arrows}
\usepackage{comment}
\usepackage[numbers]{natbib}
\usepackage[pdftex,dvipsnames]{xcolor} 

\newcommand{\carmen}[2][]{\todo[color=OliveGreen, backgroundcolor=OliveGreen!25, #1]{#2}}
\newcommand{\pelin}[2][]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue,#1]{#2}}


\newcommand{\nfa}{\textrm{NFA}}

\newcommand{\bx}{\bm{x}}
\newcommand{\bn}{\bm{n}}
\newcommand{\bv}{\bm{v}}
\newcommand{\bj}{\bm{j}}
\newcommand{\bM}{\bm{M}}
\newcommand{\bS}{\bm{S}}
\newcommand{\bphi}{\bm{\phi}}
\newcommand{\bxi}{\bm{\xi}}
\newcommand{\bunit}{\bm{I}}
\newcommand{\ba}{\bm{a}}
\newcommand{\bb}{\bm{b}}
\newcommand{\bA}{\bm{A}}
\newcommand{\bB}{\bm{B}}
\newcommand{\bu}{\bm{u}}
\newcommand{\sett}[2]{\left\{{#1}\,:~{#2}\right\}}

\newcommand{\sym}{\nabla_{sym}}
\newcommand{\as}{\nabla{as}}
\newcommand{\gd}{\nabla}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\dv}{div}



\newcommand{\dd}{\mathop{}\!\mathrm{d}}
\newcolumntype{L}{>{$}l<{$}} 

\usepackage{fancyhdr}
\usepackage{amsmath}
\usepackage{amssymb}
\pagestyle{fancy}
\thispagestyle{empty}
\fancyhead[LO]{}


\usepackage{tikz}
\usepackage{tikz-cd}
\usetikzlibrary{cd,arrows}
\tikzcdset{scale cd/.style={every label/.append style={scale=#1},
cells={nodes={scale=#1}}}}
\usetikzlibrary{decorations.markings}
\tikzset{
invisible/.style={opacity=0},
visible on/.style={alt={#1{}{invisible}}},
alt/.code args={<#1>#2#3}{%
\alt<#1>{\pgfkeysalso{#2}}{\pgfkeysalso{#3}}%
}
}
\usepackage{ragged2e}
\usepackage{tikz}
\usetikzlibrary{positioning}

\bibliographystyle{plain}
\usepackage{alltt}
\usepackage{url}
\usepackage[absolute,overlay]{textpos}
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage[english]{babel}
\usepackage{mathtools,amsmath,amsthm,amssymb}
\usepackage{extarrows}
\usepackage{transparent}
\usepackage{eucal}
\usepackage{color}
\usepackage[inkscapeformat=png]{svg}
\usepackage{graphicx}
\usepackage{placeins}       % Creates barriers for floats
\usepackage{tikz}
\usepackage[export]{adjustbox}

\usepackage{ifthen}
\usetikzlibrary{backgrounds}
\usetikzlibrary{shapes}
\usetikzlibrary{snakes}
\usetikzlibrary{patterns}        % Drawing package
\usepackage{pgfplots}
\usetikzlibrary{intersections, pgfplots.fillbetween}
\usepackage{pgfplotstable}
\usepgfplotslibrary{fillbetween}
\usepgfplotslibrary{groupplots}
\usepackage{layouts}
\usepackage{cancel}
\usepackage{multimedia}
\usepackage{qrcode}

